Topology and spectral interconnectivities of higher-order multilayer networks

Multilayer networks have permeated all the sciences as a powerful mathematical abstraction for interdependent heterogenous complex systems such as multimodal brain connectomes, transportation, ecological systems, and scientific collaboration. But describing such systems through a purely graph-theoretic formalism presupposes that the interactions that define the underlying infrastructures and support their functions are only pairwise-based; a strong assumption likely leading to oversimplifications. Indeed, most interdependent systems intrinsically involve higher-order intra- and inter-layer interactions. For instance, ecological systems involve interactions among groups within and in-between species, collaborations and citations link teams of coauthors to articles and vice versa, interactions might exist among groups of friends from different social networks, etc. While higher-order interactions have been studied for monolayer systems through the language of simplicial complexes and hypergraphs, a broad and systematic formalism incorporating them into the realm of multilayer systems is still lacking. Here, we introduce the concept of crossimplicial multicomplexes as a general formalism for modelling interdependent systems involving higher-order intra- and inter-layer connections. Subsequently, we introduce cross-homology and its spectral counterpart, the cross-Laplacian operators, to establish a rigorous mathematical framework for quantifying global and local intra- and inter-layer topological structures in such systems. When applied to multilayer networks, these cross-Laplacians provide powerful methods for detecting clusters in one layer that are controlled by hubs in another layer. We call such hubs spectral cross-hubs and define spectral persistence as a way to rank them according to their emergence along the cross-Laplacian spectra.

==> eqs/crossL.tex <==
%%% Eq: cross-Lap

For $a,b\in X_{k,l}$, the $(a,b)$-th entry of $\Lap{T}{k,l}$, for instance, with respect to the inner product defined from the weight function $w$ is given by
\begin{eqnarray*} %\label{eq:matrix-representation}
\resizebox{.9\hsize}{!}{$
  (\Lap{T}{k,l})_{a,b} = \left\{
  \begin{array}{ll}
    \frac{1}{w(a)}\deg_{TO}(a)+w(a)\deg_{TI}(a), \ {\rm if\ } a=b, \\
     \\
    \frac{w(b)}{w(d)} - \frac{w(c)}{w(a)} , \  {\rm if \ } a\neq b, \ a\outAdj{1}{c}b \ {\rm and\ } a\inAdj{1}{d}b, \\
         \ \ \ \  \ \ \ \ \ \ \  {\rm and\ have\ same\ orientation}\\
        \\ 
     \frac{w(c)}{w(a)} - \frac{w(b)}{w(d)}, \  {\rm if \ } a\neq b, \  a\outAdj{1}{c}b \ {\rm and\ } a\inAdj{1}{d}b, \\
   \ \ \ \  \ \ \  \ \ \ {\rm and\ have\ opposite\ orientations}  \\
        \\
%        \frac{w(c)}{w(b)}, & {\rm if\ } a\neq b, \  a\outAdj{1}{c}b, {\rm \ opposite\ orientations,} \\ & {\rm and\ not \ top-inner\ adjacent}, \\ 
%        & \\
%        -\frac{w(c)}{w(b)}, & {\rm if\ } a\neq b, \  a\outAdj{1}{c}b, {\rm \ same\ orientation,} \\ & {\rm and\ not \ top-inner\ adjacent}, \\ 
%        & \\
       \frac{w(b)}{w(d)}, \  {\rm if\ } a\neq b, \ a\inAdj{1}{d}b, \ {\rm same\ orientation}, \\ \ \ \ \ \ \  \ \  \  {\rm and\ not \ TO \ adjacent}, \\ 
       \\
       -\frac{w(b)}{w(d)}, \ {\rm if\ } a\neq b, \ a\inAdj{1}{d}b, \ {\rm opposite\ orientations}, \\  \ \ \  \ \ \ \ \ {\rm and\ not \ TO \ adjacent}, \\ 
        \\
       0, \ {\rm otherwise\ }.  
  \end{array}
  \right.
  $}
\end{eqnarray*}


==> tables/PCH.tex <==
%%% Table: principal cross-hub

\begin{table}[!ht]
\centering
\begin{tabular}{c|c}
%$[  v^1_0  ;   v^2_1 ]$ & $[  v^1_1  ;   v^2_1 ]$ & $[  v^1_2  ;   v^2_1 ]$ &  $[  v^1_4  ;   v^2_1 ]$ & $[  v^1_4  ;   v^2_4 ]$ & $[  v^1_6  ;   v^2_1 ]$ & $[  v^1_6  ;   v^2_2 ]$ & $[  v^1_6  ;   v^2_4 ]$ &  $[  v^1_6  ;   v^2_5 ]$ \\
%$0.4472$ & $0.4472$ & $0.4472$ & $0.4472$ & $0.0$ & $0.4472$ & $0.0$ & $0.0$ & $0.0$
$0.4472$ &  $[  v^1_0  ;   v^2_1 ]$ \\
    $0.4472$  & $[  v^1_1  ;   v^2_1 ]$ \\
    
   $0.4472$ & $[  v^1_2  ;   v^2_1 ]$ \\ 
   
  $0.4472$ &  $[  v^1_4  ;   v^2_1 ]$ \\
  
    $0.0$       & $[  v^1_4  ;   v^2_4 ]$ \\ 
    
   $0.4472$ &  $[  v^1_6  ;   v^2_1 ]$ \\
   
    $0.0$        & $[  v^1_6  ;   v^2_2 ]$  \\
    
   $0.0$       &$[  v^1_6  ;   v^2_4 ]$ \\
   $0.0$      &$[  v^1_6  ;   v^2_5 ]$
\end{tabular}%
\caption{{\bf Principal cross-hubs.} The eigenvector associated to the largest eigenvalue $\l^T_{max}=5$ of $\Lap{T}{0,0}$ for the CSB of Figure~\ref{fig:cross-betti}. $v^2_1$ is only bottom node that appears as a spectral cross-hub for $\l^T_{max}$, it is therefore the only {\em principal cross-hub} in the bottom layer with respect to the top layer, and its principal cross-hubness is $2.2360$.}
\label{tab:principal-cross-hubs}
\end{table}


==> tikz/SI_simplices.tex <==
%%%% Fig: simplices
\begin{figure}[!ht]
\centering

  \begin{tikzpicture}[scale=.8]
  %% 0-simplex
  \node[vertex] (0) at (0,0) {};
  \node at (0,0.4) {$v_0$};
  \node [below] at (0,0) { 0--simplex};
  
  %% 1-simplex
  \node[vertex] (v00) at (4,0) {};
  \node[vertex] (v01) at (6,0) {};
  \node at (4,0.4) {$v_0$};
  \node at (6,0.4) {$v_1$};
  \draw[-] (v00) -- (v01) node[midway, below] { 1--simplex};
  
  %% 2-simplex 
  \node[vertex] (v0) at (-1,-4) {};
  \node at (-1.4, -4) {$v_0$};
  
  \node[vertex] (v1) at (1, -4) {};
  \node at (1.4, -4) {$v_1$};
  
  \node[vertex] (v2) at (0,-2) {};
  \node at (0, -1.6) {$v_2$};
  
  \draw[-] (v0) -- (v1) node[midway,below] { 2--simplex}  -- (v2) -- (v0);
  %% fill the triangle
  \begin{scope}[on background layer]
  \fill [blue!20] (v0.center) -- (v1.center) -- (v2.center) -- cycle;
  \end{scope}
  
  %% 3-simplex
  \node[vertex] (vv0) at (3, -3.5) {};
  \node at (2.6, -3.5) {$v_0$};
  
  \node[vertex] (vv1) at (5, -4) {};
  \node at (5.4, -4) {$v_1$};

  
  \node[vertex] (vv2) at (6, -3) {};
  \node at (6.4, -3) {$v_2$};
  
  \node[vertex] (vv3) at (4, -2) {};
  \node at (4, -1.6) {$v_3$};
  
  \draw (vv0) -- (vv1) -- (vv3) -- (vv0);
  \draw (vv1) -- (vv2) -- (vv3) -- (vv1);
  \draw[dotted, thick] (vv0) -- (vv2);
  
  
  \begin{scope}[on background layer]
  \fill[blue!20] (vv0.center) -- (vv1.center) -- (vv3.center) -- cycle;
  \fill[blue!10] (vv1.center) -- (vv2.center) -- (vv3.center) -- cycle;
  \end{scope}
  \node at (5, -4.4) { 3--simplex};
  
\end{tikzpicture} 
\caption{Shematic illustration of simplices of dimension zero, one, two, and three in a simplicial complex.}
\label{fig:simplices}
\end{figure}  


==> tikz/SI_xLap_computations.tex <==
%%%% SI: fig - xLap-computations
\begin{figure}[!ht]
\centering
\begin{tikzpicture}[scale=0.9]
%\tikzstyle{every node}=[font=\tiny]

%%%Layers 
%%%% V_1
\begin{scope}[on background layer,opacity=0.5]
\fill[gray!20] (0,0) -- (10,0) -- (8,2) node[midway,above, black] {$ \ V_1$} -- (1,2)  -- cycle;
%%%% V_2
\fill[red!20] (0,-3) -- (10,-3) -- (8,-1)  node[midway,above, black] {$ \ V_2$} -- (1,-1) -- cycle;
\end{scope}

%%% Vertices in V1 
\node[vertex] (u0) at (7,1.5) {};
\node at (7.4,1.5) {$v^1_0$};
\node[vertex] (u1) at (6,0.5) {};
\node at (6.6,0.5) {$v^1_1$};
\node[vertex] (u2) at (4,1.2) {};
\node at (4,1.6) {$u_2$};
\node[vertex] (u3) at (2,1.5) {};
\node at (1.6,1.5) {$v^1_3$};
\node[vertex] (u4) at (3,0.5) {};
\node at (2.6,0.5) {$v^1_4$};


%%% Vertices in V2
\node[vertex] (v0) at (7,-2.5) {};
\node at (7.4, -2.5) {$v^2_0$};
\node[vertex] (v1) at (6,-1.5) {};
\node at (5.6, -1.5) {$v^2_1$};
\node[vertex] (v2) at (5,-2.5) {};
\node at (5,-2.8) {$v^2_2$};
\node[vertex] (v3) at (3,-2) {};
\node at (3, -2.4) {$v^2_3$};


% %%% Crossimplices
\draw (u0) -- (u1) -- (u2) -- (u0);
\draw (u3) -- (u2) -- (u4);

\draw (v0) -- (v1) -- (v2) -- (v0);
\draw (v2) -- (v3);

\draw[dashed] (v0) -- (u1) -- (v1);
\draw[dashed] (u2) -- (v3) -- (u3);
\draw[dashed] (u4) -- (v3);
\draw[dashed] (u3) -- (v1) -- (u4);

%% Filling the triangles
\begin{scope}[on background layer]
\fill[purple!70, opacity=0.8] (u0.center) -- (u1.center) -- (u2.center) -- cycle;
\fill[yellow!70, opacity=0.8] (v0.center) -- (v1.center) -- (v2.center) -- cycle;
\end{scope}

\begin{scope}[on background layer]
\fill[blue!15, opacity=0.8] (u1.center) -- (v0.center) -- (v1.center) -- cycle;
\fill[green!40, opacity=0.8] (u2.center) -- (v3.center) -- (u4.center) -- cycle;
\fill[green!40, opacity=0.6] (u2.center) -- (v3.center) -- (u3.center) -- cycle;
\end{scope}
%


\end{tikzpicture}

\caption{A crossimplicial bicomplex of dimension $3$.}
\label{fig:calculations-laplacians}
\end{figure}

